New Intent Discovery with Pre-training and Contrastive Learning

New intent discovery aims to uncover novel intent categories from user utterances to expand the set of supported intent classes. It is a critical task for the development and service expansion of a practical dialogue system. Despite its importance, this problem remains under-explored in the literature. Existing approaches typically rely on a large amount of labeled utterances and employ pseudo-labeling methods for representation learning and clustering, which are label-intensive, inefficient, and inaccurate. In this paper, we provide new solutions to two important research questions for new intent discovery: (1) how to learn semantic utterance representations and (2) how to better cluster utterances. Particularly, we first propose a multi-task pre-training strategy to leverage rich unlabeled data along with external labeled data for representation learning. Then, we design a new contrastive loss to exploit self-supervisory signals in unlabeled data for clustering. Extensive experiments on three intent recognition benchmarks demonstrate the high effectiveness of our proposed method, which outperforms state-of-the-art methods by a large margin in both unsupervised and semi-supervised scenarios. The source code will be available at https://github.com/zhang-yu-wei/MTP-CLNN.

==> tables/ablation_clnn2.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.85}{
\begin{tabular}{cc|ccc|ccc|ccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multicolumn{2}{c}{}&\multicolumn{3}{c}{BANKING}&\multicolumn{3}{c}{StackOverflow}&\multicolumn{3}{c}{M-CID}\\
&Methods & NMI & ARI & ACC & NMI & ARI & ACC & NMI & ARI & ACC\\
\specialrule{0.05em}{0.1em}{0.2em}
\multirow{2}{*}{25\%} 
                    % &BERT-DTC&56.05 & 20.19 &32.91 &33.38  &16.45 &30.32 &36.00 &13.64 &27.51   \\
                    % &BERT-KCL&53.85 & 20.07 &28.79 &35.47  &16.80 &32.88 &29.35 &11.58 &24.76  \\
                    % &BERT-MCL&49.46 & 15.51 &24.53 &29.44 &14.99 &31.50 &31.16 &11.30 & 26.13 \\
                    % &CDAC+&67.65& 34.88& 48.79 &74.33 &39.44 &74.30 &43.89& 19.65& 39.37\\
                    % &DAC&69.85& 37.16 & 49.67 &53.97 &36.46 &53.96 & 49.83& 27.21& 43.72  \\
                    % &\bf {Ours} &\bf88.39 & \bf 74.49 &\bf79.88 & \bf 69.46 & \bf 82.15&\bf 67.96&\bf 78.38&\bf 69.83\\
                    % & PKI \textbf{(Ours)} & 80.00&51.86&62.75 & 73.75&61.06&75.98 & 72.40&53.04&68.94 \\
                    & MTP-DAC & 81.48&55.64&66.12 & 77.22&61.42&78.60 & 77.79&62.88&77.02 \\
                    & MTP-CLNN \textbf{(Ours)} & \bf84.11&\bf61.29&\bf71.43 & \bf79.68&\bf70.17&\bf83.77 & \bf80.24&\bf66.77&\bf79.20 \\
                    %&\bf {Ours} &\bf88.44 & \bf 80.73 &\bf68.74 & \bf 65.64 & \bf 74.11&\bf 69.93&\bf 87.08&\bf 79.67\\
\specialrule{0.05em}{0.1em}{0.2em}
\multirow{2}{*}{50\%} 
                    % &BERT-DTC& 69.68&35.98&48.87 & 53.94&36.79&51.78 & 51.90&28.94&44.70\\
                    % &BERT-KCL& 62.86&30.16&40.81 & 57.63&41.90&56.58 & 42.48&22.83&38.11\\
                    % &BERT-MCL& 62.50&29.80&42.28 & 49.49&35.96&53.16 & 41.50&21.46&37.99\\
                    % &CDAC+& 70.62&38.61&51.97 & 76.18&41.92&76.30 & 50.47&26.01&46.65\\
                    % &DAC& 76.41&47.28&59.32 & 70.78&56.44&73.76 & 63.27&43.52&57.19 \\
                    % &\bf {Ours}&\bf 85.44 &\bf 84.17 &\bf 78.17 &\bf 79.16 & \bf 74.91&\bf 77.34&\bf74.19&\bf75.12\\
                    %&\bf {Ours}&\bf 88.33 &\bf 86.67 &\bf 75.08 &\bf 78.55 & \bf 72.69&\bf 79.21&\bf81.05&\bf79.73\\
                    % &PKI \textbf{(Ours)}& 82.92&58.46&68.29 & 77.11&66.45&79.28 & 72.40&53.04&68.94 \\
                    &MTP-DAC& 83.43&59.78&70.42 & 78.91&67.37&81.27 & 78.17&63.41&77.68 \\
                    &MTP-CLNN \textbf{(Ours)}& \bf85.62&\bf64.93&\bf75.23 & \bf81.03&\bf73.02&\bf85.64 & \bf79.48&\bf65.71&\bf77.85 \\
\specialrule{0.05em}{0.1em}{0.2em}
\multirow{2}{*}{75\%} 
                    % &BERT-DTC& 74.51&44.57&57.34 & 67.02&55.14&71.14 & 60.82&38.62&55.42 \\
                    % &BERT-KCL& 72.18&44.29&58.70 & 70.38&57.98&71.50 & 54.22&34.60&52.15 \\
                    % &BERT-MCL& 74.41&48.08&61.57 & 67.72&55.78&70.82 & 51.33&31.22&50.77 \\
                    % &CDAC+& 71.76&40.68&53.46 & 76.68&43.97&75.34 & 55.06&32.52&53.70 \\
                    % &DAC& 79.99&54.57&65.87 & 75.31&60.02&78.84 & 71.41&54.22&69.11 \\
                    % &\bf {Ours}&\bf85.08 & 86.30 &\bf81.08 & \bf85.11 &\bf79.32 &84.66&\bf77.14&79.53\\
                    %&\bf {Ours}&\bf88.08 & \bf89.43 &\bf81.71 & \bf85.85 &\bf81.07 &\bf86.98&\bf80.24&\bf82.75\\
                    % &PKI \textbf{(Ours)}& 85.17&64.37&74.20 & 80.70&71.68&83.74 & 80.95&69.27&80.92 \\
                    &MTP-DAC& 85.78&65.28&75.43 & 80.89&71.17&84.20 & 80.94&68.27&80.89 \\
                    &MTP-CLNN \textbf{(Ours)}& \bf87.52&\bf70.00&\bf79.74 & \bf82.56&\bf75.66&\bf87.63 & \bf83.75&\bf73.22&\bf84.36 \\
\specialrule{0.1em}{0.1em}{0.2em}
\end{tabular}
}
\caption{\label{tab:ablation_clnn2}
Comparison with a stronger baseline on semi-supervised NID where $\text{LAR}=10\%$.
%Overall accuracy and macro f1-score for unknown intent detection with different proportion of seen classes. For each setting, the best result is marked in bold. 
% For the 75\% setting, the top 2 results for each metric are marked in bold.
}
\end{table*}
